Discrete Symmetries in the MSSM

The use of discrete symmetries, especially abelian ones, in physics beyond the standard model of particle physics is discussed. A method is developed how a general, abelian, discrete symmetry can be obtained via spontaneous symmetry breaking. In addition, anomalies are treated in the path integral approach with special attention to anomaly cancellation via the Green-Schwarz mechanism. All this is applied to the minimal supersymmetric standard model. A unique Z_4^R symmetry is discovered which solves the \mu-problem as well as problems with proton decay and allows to embed the standard model gauge group into a simple group, i.e. the Z_4^R is compatible with grand unification. Also the flavor problem in the context of minimal flavor violation is addressed. Finally, a string theory model is presented which exhibits the mentioned Z_4^R symmetry and other desirable features.

==> titlepage/titlepage.tex <==
% \thispagestyle{empty}
\pagestyle{empty}
\pagenumbering{Roman}


% \newpage
% \phantom{x}
% \newpage

% \begin{center}
%  \Huge{Physik-Department}
%  \vspace{5mm}
%  \end{center}
%  \begin{figure}[h]
%   \centering
%   \includegraphics[scale=3]{titlepage/PHLogo.eps}
%  \end{figure}
%  \begin{center}
%  \vfill
%  \Huge{\textbf{Discrete Symmetries in the MSSM}}
% 
%  \vfill
%  \huge{Dissertation von}
% 
%  \vspace{1cm}
%  \Huge{Roland Schieren}
% 
%  \vfill
%   \begin{figure}[h]
%   \centering
%   \includegraphics[scale=2]{titlepage/TUMLogo.eps}
%  \end{figure}
%  Technische Universität München
% \end{center}

% \setcounter{page}{1}


\begin{tabular}{lcr}
\parbox[t]{0.55\textwidth}{
\begin{center}
 {\large\bfseries TECHNISCHE UNIVERSITÄT MÜNCHEN}\\
 Physik-Department\\
 Institut für Theoretische Physik T30e\\
 Univ.-Prof. Dr. Michael Ratz
\end{center}}
&\parbox[t]{0.15\textwidth}{ \hfill} &
\parbox[t]{0.15\textwidth}{
\begin{center}
\includegraphics[height=1.6cm]{titlepage/TUMLogo.eps}
\end{center}}
\end{tabular}\\[1.3cm]

\begin{center}
 {\Huge\bfseries Discrete Symmetries in the MSSM\\[1.cm]}
 {\LARGE Roland Schieren}\\[2.5cm]
\end{center}

\noindent
Vollst\"andiger Abdruck der von der Fakultät für Physik der
Technischen Universität München zur Erlangung des akademischen
Grades eines
\vspace{4mm}
\begin{center}
 {\bfseries Doktors der Naturwissenschaften (Dr. rer. nat.)}
\end{center}
\vspace{3mm}
genehmigten Dissertation.

\vspace{1.5cm}

\begin{tabular}{lll}
                          &   & \hspace{6cm}\ \\
Vorsitzender:              &   & Univ.-Prof. Dr. Lothar Oberauer \\[3mm]
Pr\"ufer der Dissertation: &1. & Univ.-Prof. Dr. Michael Ratz\\[3mm]
                          &2. & Univ.-Prof. Dr. Alejandro Ibarra\\[3mm]
                         
\end{tabular}

\vfill
\noindent
Die Dissertation wurde am 4.~November 2010 bei der
Technischen Universit\"at 
M\"un\-chen ein\-ge\-reicht und durch die Fakult\"at f\"ur Physik 
am 2.~Dezember 2010 angenommen.


%\newpage



